Hawkeye: Hectometer-range Subcentimeter Localization for Large-scale mmWave Backscatter

Accurate localization of a large number of objects over a wide area is one of the keys to the pervasive interaction with the Internet of Things. This paper presents Hawkeye, a new mmWave backscatter that, for the first time, offers over (i) hundred-scale simultaneous 3D localization at (ii) subcentimeter accuracy for over an (iii) hectometer distance. Hawkeye generally applies to indoors and outdoors as well as under mobility. Hawkeye tag's Van Atta Array design with retro-reflectivity in both elevation and azimuth planes offers 3D localization and effectively suppresses the multipath. Hawkeye localization algorithm is a lightweight signal processing compatible with the commodity FMCW radar. It uniquely leverages the interplay between the tag signal and clutter, and leverages the spetral leakage for fine-grained positioning. Prototype evaluations in corridor, lecture room, and soccer field reveal 6.7 mm median accuracy at 160 m range, and simultaneously localizes 100 tags in only 33.2 ms. Hawkeye is reliable under temperature change with significant oscillator frequency offset.

==> 2.motivation.tex <==
\section{Motivation}

















==> 5.implementation.tex <==
%-------------------------------------------------------------------------------
% \iffalse
% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lll}
% \hline
% \textbf{Component}        & \textbf{Lines of Code (LoC)} & \textbf{Changed} \\ \hline
% \textbf{\sys PDCP}  &  XX lines of C++         & - (XX)    \\
% \textbf{\sys RLC} & XX lines of C++         & - (XX)  \\
% \textbf{\sys MAC} & XX lines of C++   & XX\% (XX)  \\ \hline
% \end{tabular}
% }
% \vspace{-10pt}
% \textbf{\caption{\sys implementation (Lines of Code)}}
% \vspace{-18pt}
% %\vspace{-25pt}
% \label{tab:impl}
% \end{table}
% \fi
% \newpage



\begin{figure}[t!]
\vspace{-0.2cm}
\centering
    \subfigure[]{\includegraphics[width=0.34\columnwidth]{figures/tags111.jpg}}
    %\hfill
    \hspace{0.1in}
    \subfigure[]{\includegraphics[width=0.39\columnwidth]{figures/tag_nocase.jpg}}
    \subfigure[]{\includegraphics[width=0.57\columnwidth]{figures/S11_ver2.eps}}
    \hspace{0.1in}
    \subfigure[]{\includegraphics[width=0.35\columnwidth]{figures/Switch_Circuit.jpg}}
    %\hfill
    % \hspace{0.2mm}
    
    \vspace{-3mm}
    \caption{(a) 6 of our mmWave tags inside the aluminum casing. (b) Our mmWave tag board. (c) The S(11) parameter of our tag at switch close. (d) The tag's circuit diagram.}
    \label{fig:base}
     \vspace{+5mm}
\end{figure}

\newpage
\section{Implementation}\label{sec:implementation}

This section presents implementation details.

% \begin{figure}[h!]
% \centering
% % \vspace{-0.2cm}
% \includegraphics[width=0.98\columnwidth]{figures/uc.jpg}
% \vspace{-3.5mm}
% \caption{(a) Baseline mmWave backscatter prototype. (b) Van Atta backscatter prototype.}\label{fig:tags}
% \vspace{-0.3cm}
% \end{figure}



% \begin{figure}[h!]
%   \begin{center}
%     \begin{subfigure}{0.95\columnwidth}
%       \includegraphics[width=\columnwidth]{figures/uc.jpg}
%     \end{subfigure}
%     \hspace{-0.0cm} % spacing between sub-figures. Minus value to make them closer (if too large blank)
%     \begin{subfigure}{0.4\columnwidth}
%       \includegraphics[width=\columnwidth]{figures/uc.jpg}
%     \end{subfigure}
%     \hspace{-0.0cm} % spacing between sub-figures
%     \begin{subfigure}{0.55\columnwidth}
%       \includegraphics[width=\columnwidth]{figures/uc.jpg}
%     \end{subfigure}
%   \end{center}
%   \vspace{-0.3cm} % Spacing between figures and the main caption. Minus value to make them closer (if too large blank)
%   \caption{(a)Baseline mmWave circuit diagram. (b) Photo of baseline mmWave circuit. (c) The S(11) parameters of switch close. \kangmin{erase switch open part, explain by words.}}
%   \label{fig:circuit_tag1_s11} % Or reference the whole figure
%   \vspace{-0.3cm} % Spacing below the caption and the texts. Minus value to make them closer (if too large blank)
% \end{figure}

% \begin{figure*}[h!]
% \vspace{-0.4cm}
% \centering
%     \subfigure[setup wide]{\includegraphics[width=1.58\columnwidth]{figures/wide_setup_5.jpg}}
%     \hfill
%     % \hspace{0.2mm}
%     \subfigure[Heatmap]{\includegraphics[width=0.5\columnwidth]{figures/heatmap5.jpg}}
%     \subfigure[]{\includegraphics[width=1.5\columnwidth]{figures/tags_photo2.jpg}}
%     \subfigure[]{\includegraphics[width=0.5\columnwidth]{figures3/many_tags_BER_tall.eps}}
%     \vspace{-3mm}
%     \caption{Setup and heatmap.}
%     \label{fig:setup_heatmap}
%     \vspace{-5mm}
%     % \subfigure[BER]{\includegraphics[width=2\columnwidth]{figures3/many_tags_BER_short.eps}}
% \end{figure*}


% \begin{figure*}
%   \begin{center}
%     \begin{subfigure}{1.49\columnwidth}
%       \includegraphics[width=\columnwidth]{figures/uc.jpg}
%       \caption{setup wide}
%     \end{subfigure}
%     \hspace{-0.0cm} % spacing between sub-figures. Minus value to make them closer (if too large blank)
%     \begin{subfigure}{0.5\columnwidth}
%       \includegraphics[width=\columnwidth]{figures/uc.jpg}
%       \caption{Heatmap4}
%     \end{subfigure}
%   \end{center}
  
%   \vspace{-0.3cm} % Spacing between figures and the main caption. Minus value to make them closer (if too large blank)
  
%   \caption{Setup and Hitmap}
%   \label{fig:setup_hitmap} % Or reference the whole figure
%   \vspace{-0.3cm} % Spacing below the caption and the texts. Minus value to make them closer (if too large blank)
% \end{figure*}


\subsection{\ours Tag Prototype}

Figure~\ref{fig:base}(a)-(b) show the prototype of 24GHz \ours tag implemented on Rogers RO4003C substrate with MACOM MASW-011105 GaAs SPDT RF switch. The RFC port of the switch is connected to the commodity 24GHz 17dBi microstrip array antenna, and the RF1 / RF2 ports are connected to 50 $\Omega$ matched ground and open. Figure~\ref{fig:base} (c) depicts the measurement result of the return loss (S(11)) at non-reflective state (i.e., matched ground). The return loss of flat -9.5dB at reflective state, leading to a difference of over 20dB between the switch states. For tag control signal, either Altera TerasIC T-Core P0633 FPGA board or Arduino Uno were used. The form factor is $40.3\times30.1$mm.

\vspace{0.1in}\noindent \textbf{Power Consumption.} The tag uses MACOM RF switch with 5$\mu W$ power consumption. For power consumption analysis, we design a 2-FSK backscatter tag and simulate an IC for the control board, as shown in Figure~\ref{fig:base}(d). A ring oscillator and modulator circuit with a power consumption of 2$\mu W$ are used for frequency shift and control logic. The total power consumption is 7$\mu W$ (well below the 33 $\mu W$ energy harvesting~\cite{zhang2016hitchhike}), which can operate battery-free, or with a coin cell battery of 1000 $mAh$ for 48.9 years.



\begin{figure}[t!]
\centering
\subfigure[]{\includegraphics[width=0.34\columnwidth]{figures/t22.jpg}}
\subfigure[]{\includegraphics[width=0.64\columnwidth]{figures3/polar_2.eps}}
\vspace{-3mm}
\caption{(a) Prototype tag with Van Atta array antenna, and (b) beam pattern (retro-reflectivity)}\label{fig:va}
\vspace{-4mm}
\end{figure}

\begin{figure}[t!]
\centering
 \subfigure[]{\includegraphics[width=0.55\columnwidth]{figures/X4.jpg}}
 \subfigure[]{\includegraphics[width=0.4\columnwidth]{figures/X5.jpg}}
\vspace{-3mm}
\caption{\ours custom reader backend (a) schematic diagram and (b) snapshot.}\label{fig:customgateway}
\vspace{-5mm}
\end{figure}




\begin{figure}[h!]
\centering
\subfigure[]{\includegraphics[width=0.35\columnwidth]{figures/r11.jpg}}
\subfigure[]{\includegraphics[width=0.55\columnwidth]{figures3/polar_1.eps}}
\vspace{-3mm}
\caption{(a) \ours reader implemented on Eval-Tinyrad, and (b) the single Tx antenna omni-directional beam pattern}\label{fig:omni}
\vspace{-5mm}
\end{figure}


%%%%
\begin{figure*}[h!]
\centering
    \begin{minipage}[b]{1.25\columnwidth}
        \includegraphics[width=\columnwidth]{figures/wide_set_2.jpg}
        \vspace{-6mm}
        \caption{\ours evaluation in a practical office setting of approx 10 x 10m. Radar is omni-directional. Some tags are enclosed in a wooden cabinet (tag 14), packaged in a cardboard box (tag 15), hidden behind a wooden bookcase (tag 16), and obstructed by metal partitions (tag 18).}
        \label{fig:setup}
    \end{minipage} \quad
    \begin{minipage}[b]{0.7\columnwidth}
        \includegraphics[width=\columnwidth]{figures/Wide_set_3_fix1.jpg}
        \vspace{-6mm}
        \caption{(a) Signal strength and (b) BER of the tag with a single omni-directional radar. Signal strength as low as -103.6dBm achieves < 10\% BER}
        \label{fig:heatmap}
    \end{minipage}
    % \vspace{-3mm}
    % \caption{Setup and heatmap. \kangmin{split this into two figures}}
    \vspace{-3mm}
\end{figure*}



\vspace{0.1in}\noindent \textbf{Implementation Cost.} The tag can be produced at a reasonable price of 40.528 USD. This consists of Macom MASW-011105 switch (20 USD), Rogers RO4003C substrate (0.028 USD considering the required substrate size), and an Arduino Uno (20 USD) with a signal inverter (0.5 USD) for control. Figure~\ref{fig:va} presents our Van Atta prototype tag, built on EVAL-ADRF5026 board and commodity 24GHz antennas. Figure~\ref{fig:va} depicts beam pattern measurement of the Van Atta tag showing the retro-reflective operation of over -20dB over the full 180 degrees of incident angle. \ours 60GHz tag uses V-Band Reflective SPST PIN Diode Switch (Eravant), with WR-15 Waveguide Horn Antenna (Pasternack) and WR-15 WAVEGUIDE OPEN (Eravant).

% \begin{comment}
% \begin{figure*}[h!]
% \vspace{-0.4cm}
% \centering
%     \subfigure[Setup and heatmap.]{\includegraphics[width=1.15\columnwidth]{figures/wide_set2.jpg}}
%     \subfigure[BER]{\includegraphics[width=0.65\columnwidth]{figures3/many_tags_BER_all.eps}}
%     \vspace{-3mm}
%     \caption{Setup and heatmap.}
%     \label{fig:setup_heatmap}
%     \vspace{-5mm}
% \end{figure*}
% \end{comment}



% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\columnwidth]{figures/X3.jpg}
% \vspace{-3mm}
% \caption{\ours custom gateway.}\label{fig:customgateway}
% \vspace{-5mm}
% \end{figure}


\vspace{0.1in}
\subsection{\ours Reader Implementation}\label{sec:commodity}
Implementation if \ours on commodity radars only requires signal processing, without any change to the hardware. Implementation on 24GHz commodity radars are on Distance2Go (Infineon) and EVAL-Tinyrad (Analog Devices), while the 60GHz reader uses mmWaveICBoost , IWR6843ISK antenna and DCA1000EVM interface boards. The readers provide real-time raw data, but does not allow the inter-chirp interval to be reduced to zero. To address this, HD-FMCW is implemented at the receiver side, by reconstructing the received signal and compensating the phase offset. The chirp signals are carefully concatenated to keep the phase continuity of the tag signal, where the inter-chirp interval is known and set using the customized chirp parameters. SDR-based testbed is implemented for in-depth analysis. The 24GHz testbed in Figure~\ref{fig:customgateway} uses two USRP X310s for Tx and Rx, operating through up and down converters (EVAL-ADMV1013, EVAL-ADMV1014) quadrupled from 6GHz external LO. 




% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures3/many_tags_BER_short.eps}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures3/many_tags_BER_tall.eps}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{comment}

% % Old subfigure package

% \begin{figure}[t!]
%   \subfigbottomskip = 0cm
%   \subfigcapmargin = 3pt
%   \begin{center}
%     \subfigure[] % You can reference each sub-figures
%     {
%       % 0.66 Columnwidth * 3 = 1.98 Columnwidth
%       % Control 0.66/0.66/0.66 in each sub-figure to resize
%       % Make sure the sum of three size is less then 2 Columnwidth
%       % You can also specify the height like ", height=6cm". But this may make the image to distort if not calculated correctly. Just use the width only!
%       \includegraphics[width=0.85\columnwidth]{figure5/circuit.jpg}
%     }
%     \hspace{-0.3cm} % spacing between sub-figures. Minus value to make them closer (if too large blank)
%     \subfigure[]
%     {
%       \includegraphics[width=0.35\columnwidth]{figure5/tag1.jpg}
%     }
%     \hspace{-0.3cm} % spacing between sub-figures
%     \subfigure[]
%     {
%       \includegraphics[width=0.45\columnwidth]{figure5/S11.eps}
%     } 
%   \end{center}
%   \vspace{-0.3cm} % Spacing between figures and the main caption. Minus value to make them closer (if too large blank)
%   \caption{(a)Baseline mmWave circuit diagram. (b) Photo of baseline mmWave circuit. (c) The S(11) parameters of switch close and open.}
%   \label{fig:ex1} % Or reference the whole figure
%   \vspace{-0.3cm} % Spacing below the caption and the texts. Minus value to make them closer (if too large blank)
% \end{figure}

% \begin{figure*}[h!]
%   \subfigbottomskip = 0cm
%   \subfigcapmargin = 3pt
%   \begin{center}
%     \subfigure[Caption1 \label{fig:ex1_1}] % You can reference each sub-figures
%     {
%       % 0.66 Columnwidth * 3 = 1.98 Columnwidth
%       % Control 0.66/0.66/0.66 in each sub-figure to resize
%       % Make sure the sum of three size is less then 2 Columnwidth
%       % You can also specify the height like ", height=6cm". But this may make the image to distort if not calculated correctly. Just use the width only!
%       \includegraphics[width=1.49\columnwidth]{figure5/setup_wide.jpg}
%     }
%     \hspace{-0.3cm} % spacing between sub-figures. Minus value to make them closer (if too large blank)
%     % \subfigure[Caption2 \label{fig:ex1_2}]
%     % {
%     %   \includegraphics[width=0.66\columnwidth]{figure4/pene_range.jpg}
%     % }
%     % \hspace{-0.3cm} % spacing between sub-figures
%     \subfigure[Caption3 \label{fig:ex1_3}]
%     {
%       \includegraphics[width=0.5\columnwidth]{figure5/heatmap4.jpg}
%     } 
%   \end{center}
%   \vspace{-0.3cm} % Spacing between figures and the main caption. Minus value to make them closer (if too large blank)
%   \caption{Main Caption}
%   \label{fig:ex1} % Or reference the whole figure
%   \vspace{-0.3cm} % Spacing below the caption and the texts. Minus value to make them closer (if too large blank)
% \end{figure*}

% \end{comment}




==> 8.discussion.tex <==
%-------------------------------------------------------------------------------
\section{Discussions}

\noindent\textbf{Case for QoS support by legacy LTE/5G.} 


\noindent\textbf{Case for handovers.} 


\noindent\textbf{Case for uplink scheduling.} 


\noindent\textbf{Online adaptation of the parameters.} 

%-------------------------------------------------------------------------------

==> discussion.tex <==
% \begin{figure*}[h!]
% \vspace{-0.4cm}
% \centering
%     \subfigure[setup wide]{\includegraphics[width=1.48\columnwidth]{figures/setup_wide.jpg}}
%     \hfill
%     % \hspace{0.2mm}
%     \subfigure[Heatmap]{\includegraphics[width=0.6\columnwidth]{figures/heatmap.jpg}}
%     \vspace{-3mm}
%     \caption{Setup and heatmap.}
%     \label{fig:setup_heatmap}
%     \vspace{-5mm}
% \end{figure*}

% \begin{figure*}[h!]
% \vspace{-0.4cm}
% \centering
%     \subfigure[First]{\includegraphics[width=0.214\columnwidth]{figures/ttt.jpg}}
%     \hfill
%     \subfigure[First]{\includegraphics[width=0.35\columnwidth]{figures/r1.jpg}} 
%     \hfill
%     % \hspace{-3mm}
%     \subfigure[First]{\includegraphics[width=0.35\columnwidth]{figures/r2.jpg}}
%     \hfill
%     % \hspace{-3mm}
%     \subfigure[First]{\includegraphics[width=0.35\columnwidth]{figures/r3.jpg}} 
%     \hfill
%     % \hspace{-3mm}
%     \subfigure[First]{\includegraphics[width=0.503\columnwidth]{figures/X1.jpg}}
%   \vspace{-3mm}
%   \caption{(a)Clutter noise rejection at outdoor. (b) Clutter noise rejection at hallway. (c) Clutter noise rejection at office. (d) Snapshot of each experiment scenarios.}
%   \label{fig:clutter_noise} % Or reference the whole figure
%   \vspace{-3mm}
  
% \end{figure*}

\section{Discussion}

In this section, we discuss the potential capacity of \ours including the downlink support and location based services, as well as the effect of near-far problem on \ours.

\vspace{0.1in}\noindent \textbf{Downlink Support.}
The downlink is transparently supported at \ours, as the tags operating in \ours network is sure to receive the downlink signal as a part of the interrogation signal. Downlink can be easily achieved through known techniques such as power detection with on-off keying. The implementation of downlink opens many additional opportunities, such as the support of data acknowledgements or radar-tag synchronization for additional reliability to \ours communication. Furthermore, tag channel allocation (discussed at (\textsection\ref{sec:channelalloc})) can be dynamically supported to maintain optimal channel utilization under varying environments.

\vspace{0.1in}\noindent \textbf{Location-based Services.}
\ours exploits the large mmWave bandwidth by utilizing the physical distance between the radar and the tag, where the distance is reflected as the channel allocation of the tag. This implies that the location of each tag can be recognized in the process of demodulation. As a result, \ours can be modified to support location-based services (e.g., smart factory or warehouse) on top of \ours communication and network.

\vspace{0.1in}\noindent \textbf{The near-far problem.}
The near-far problem is often discussed in concurrent backscatter systems \cite{hessar19}, where the backscatter signals from a nearby tag can overpower a farther concurrent tag. Whereas the location-based channel allocation liberate \ours from the near-far problem, as the tags at similar communication distances (and thus similar signal strengths) are allocated adjacent channels.

% 2D localization with mimo antenna
% if we have downlink (variable chirp number, duration). increase bin such that collision probability is under the threshold.

% \songmin{radar-tag chirp asynchronization, near-far problem.}
